What Does a ProcGen Generalization Gap Measure? Action Rules, Residual Entropy, and the Missing Random Floor

A generalization gap in reinforcement learning, return on training levels minus return on held-out levels, is usually reported without a reference point. We argue that it should be read against a measured random floor: the return of a uniform-random policy on the same levels under the same evaluation harness. On eight ProcGen environments with PPO at a compute-limited budget (8M steps, 16 parallel environments; three games extended to 25M), the floor changes what standard numbers mean. The test-time action rule decides which policy is measured: in miner, the sampled policy scores 5.1x the floor on held-out levels while its argmax scores below it in every run, and greedy evaluation places two environments significantly below the floor. Used as a convergence diagnostic, raw policy entropy flags six of eight environments, but 32-66% of that entropy lies on actions with identical effects; against the floor, five of eight sampled policies are clearly above it on held-out levels and heist's is not distinguishable from it. An audit of twelve ProcGen codebases finds that nine sample test-time actions with no explicit choice at the evaluation call site. We recommend that every reported gap state its action rule, seed its evaluation and specify its tests before analysis, and report the floor on both level sets.

==> numbers.tex <==
% generated by scripts/tmlr_numbers.py from results/tmlr/ -- do not edit
\makeatletter
\newcommand{\N}[1]{\@ifundefined{num@#1}{\textbf{??#1??}\PackageWarning{numbers}{undefined number #1}}{\@nameuse{num@#1}}}
\@namedef{num@H.fruitbot.8M.share}{66}
\@namedef{num@H.miner.8M}{2.087}
\@namedef{num@H.miner.8M.first}{1.726}
\@namedef{num@H.miner.8M.pct}{77.1}
\@namedef{num@H.miner.8M.probe}{2.083}
\@namedef{num@H.starpilot.25M.first}{2.145}
\@namedef{num@H.starpilot.25M.probe}{1.583}
\@namedef{num@coinrun.8M.g.test}{3.57}
\@namedef{num@coinrun.8M.s.test}{5.72}
\@namedef{num@count.above.8M.s}{5}
\@namedef{num@count.above.8M.s.word}{five}
\@namedef{num@count.below.8M.g}{2}
\@namedef{num@count.below.8M.g.word}{two}
\@namedef{num@count.game.8M}{3}
\@namedef{num@count.game.8M.word}{three}
\@namedef{num@count.raw.8M.word}{six}
\@namedef{num@count.state.8M}{2}
\@namedef{num@count.state.8M.word}{two}
\@namedef{num@count.v1atbelow.8M.g}{3}
\@namedef{num@d.bigfish.8M.s.test.z}{$+$2.6}
\@namedef{num@d.fruitbot.8M.s.test.ph}{$2.9\times10^{-11}$}
\@namedef{num@d.heist.25M.s.test}{$-$0.15}
\@namedef{num@d.heist.25M.s.test.hi}{$+$0.44}
\@namedef{num@d.heist.25M.s.test.label}{not distinguishable}
\@namedef{num@d.heist.25M.s.test.lo}{$-$0.73}
\@namedef{num@d.heist.25M.s.train.ph}{$8.7\times10^{-23}$}
\@namedef{num@d.heist.8M.s.test}{$-$0.27}
\@namedef{num@d.heist.8M.s.test.hi}{$+$0.31}
\@namedef{num@d.heist.8M.s.test.lo}{$-$0.86}
\@namedef{num@d.heist.8M.s.test.ptost}{0.45}
\@namedef{num@d.heist.8M.s.train.ph}{0.075}
\@namedef{num@d.heist.8M.s.train.u}{0.88}
\@namedef{num@d.miner.8M.g.test.n}{6}
\@namedef{num@d.miner.8M.g.test.ph}{$2.6\times10^{-4}$}
\@namedef{num@d.miner.8M.s.test.n}{6}
\@namedef{num@dodgeball.8M.g.test}{0.82}
\@namedef{num@dodgeball.8M.s.test}{1.09}
\@namedef{num@enc.heist.25M.s.test.fpn.z}{$+$0.6}
\@namedef{num@enc.heist.25M.s.test.impala.z}{$-$1.4}
\@namedef{num@encd.heist.25M.g.gap.p}{0.002}
\@namedef{num@encd.heist.25M.g.gap.u}{1.37}
\@namedef{num@encd.heist.25M.s.gap.p}{$5.7\times10^{-4}$}
\@namedef{num@encd.heist.25M.s.gap.u}{1.06}
\@namedef{num@encd.heist.25M.s.share}{36}
\@namedef{num@encd.starpilot.25M.s.gap.p}{0.010}
\@namedef{num@encd.starpilot.25M.s.test.p}{0.90}
\@namedef{num@encpd.heist.25M.s.gap.pmax}{0.019}
\@namedef{num@encpd.heist.25M.s.test.pmax}{0.27}
\@namedef{num@encpd.heist.25M.s.test.pmin}{0.028}
\@namedef{num@floor.coinrun.test}{3.28}
\@namedef{num@floor.heist.test}{3.15}
\@namedef{num@floor.heist.train}{3.54}
\@namedef{num@floor.miner.test}{1.17}
\@namedef{num@gap.heist.25M.g.u}{2.62}
\@namedef{num@gap.heist.25M.s.u}{3.94}
\@namedef{num@gap.heist.8M.g.u}{0.71}
\@namedef{num@gap.heist.8M.s.u}{1.54}
\@namedef{num@gap.miner.8M.g.u}{0.61}
\@namedef{num@gap.miner.8M.s.u}{1.55}
\@namedef{num@gap.starpilot.25M.s}{$+$2.11}
\@namedef{num@gap.starpilot.25M.s.hi}{$+$2.77}
\@namedef{num@gap.starpilot.25M.s.lo}{$+$1.39}
\@namedef{num@gap.starpilot.8M.s}{$-$0.23}
\@namedef{num@gap.starpilot.8M.s.hi}{$+$0.48}
\@namedef{num@gap.starpilot.8M.s.lo}{$-$0.79}
\@namedef{num@gd.heist.25M}{$+$1.32}
\@namedef{num@gd.heist.25M.hi}{$+$1.72}
\@namedef{num@gd.heist.25M.lo}{$+$0.94}
\@namedef{num@gd.heist.8M}{$+$0.83}
\@namedef{num@gd.heist.8M.hi}{$+$1.13}
\@namedef{num@gd.heist.8M.lo}{$+$0.49}
\@namedef{num@gd.heist.8M.p}{0.007}
\@namedef{num@heist.25M.s.test}{3.00}
\@namedef{num@heist.25M.s.train}{6.94}
\@namedef{num@heist.8M.s.test}{2.88}
\@namedef{num@heist.8M.s.train}{4.42}
\@namedef{num@miner.8M.g.test}{0.60}
\@namedef{num@miner.8M.s.test}{5.93}
\@namedef{num@ratio.miner.8M.s.test}{5.1}
\@namedef{num@rd.bossfight.8M.test.kg}{5}
\@namedef{num@rd.dodgeball.8M.test.p}{0.066}
\@namedef{num@rd.heist.8M.test.u}{2.43}
\@namedef{num@share.max.8M}{66}
\@namedef{num@share.min.8M}{32}
\@namedef{num@succ.heist.8M.g.test}{5}
\@namedef{num@succ.heist.8M.s.test}{29}
\@namedef{num@succ.heist.floor.test}{32}
\makeatother


==> numbers_carried.tex <==
% generated by scripts/tmlr_carry.py (appendix representation diagnostics)
\makeatletter
\@namedef{num@cka.starpilot.within_impala.8M}{0.020}
\@namedef{num@cka.starpilot.within_impala.8M.sd}{0.001}
\@namedef{num@cka.starpilot.cross_train.8M}{0.703}
\@namedef{num@cka.starpilot.cross_train.8M.sd}{0.063}
\@namedef{num@cka.starpilot.cross_test.8M}{0.731}
\@namedef{num@cka.starpilot.cross_test.8M.sd}{0.038}
\@namedef{num@cka.starpilot.within_fpn.8M}{0.020}
\@namedef{num@cka.starpilot.within_fpn.8M.sd}{0.007}
\@namedef{num@cka.fruitbot.within_impala.8M}{0.144}
\@namedef{num@cka.fruitbot.within_impala.8M.sd}{0.012}
\@namedef{num@cka.fruitbot.cross_train.8M}{0.543}
\@namedef{num@cka.fruitbot.cross_train.8M.sd}{0.026}
\@namedef{num@cka.fruitbot.cross_test.8M}{0.458}
\@namedef{num@cka.fruitbot.cross_test.8M.sd}{0.042}
\@namedef{num@cka.fruitbot.within_fpn.8M}{0.042}
\@namedef{num@cka.fruitbot.within_fpn.8M.sd}{0.012}
\@namedef{num@cka.starpilot.within_impala.25M}{0.022}
\@namedef{num@cka.starpilot.within_impala.25M.sd}{0.004}
\@namedef{num@cka.starpilot.within_fpn.25M}{0.021}
\@namedef{num@cka.starpilot.within_fpn.25M.sd}{0.009}
\@namedef{num@cka.starpilot.cross_train.25M}{0.757}
\@namedef{num@cka.starpilot.cross_train.25M.sd}{0.065}
\@namedef{num@cka.starpilot.cross_test.25M}{0.783}
\@namedef{num@cka.starpilot.cross_test.25M.sd}{0.058}
\@namedef{num@cka.fruitbot.within_impala.25M}{0.110}
\@namedef{num@cka.fruitbot.within_impala.25M.sd}{0.012}
\@namedef{num@cka.fruitbot.within_fpn.25M}{0.085}
\@namedef{num@cka.fruitbot.within_fpn.25M.sd}{0.009}
\@namedef{num@cka.fruitbot.cross_train.25M}{0.518}
\@namedef{num@cka.fruitbot.cross_train.25M.sd}{0.022}
\@namedef{num@cka.fruitbot.cross_test.25M}{0.533}
\@namedef{num@cka.fruitbot.cross_test.25M.sd}{0.023}
\@namedef{num@cka.heist.within_impala.25M}{0.104}
\@namedef{num@cka.heist.within_impala.25M.sd}{0.024}
\@namedef{num@cka.heist.within_fpn.25M}{0.068}
\@namedef{num@cka.heist.within_fpn.25M.sd}{0.009}
\@namedef{num@cka.heist.cross_train.25M}{0.593}
\@namedef{num@cka.heist.cross_train.25M.sd}{0.048}
\@namedef{num@cka.heist.cross_test.25M}{0.678}
\@namedef{num@cka.heist.cross_test.25M.sd}{0.041}
\@namedef{num@ctl.starpilot.impala.reported}{0.020}
\@namedef{num@ctl.starpilot.impala.perm_mean}{0.001}
\@namedef{num@ctl.starpilot.impala.analytic}{0.001}
\@namedef{num@ctl.starpilot.impala.A}{0.008}
\@namedef{num@ctl.starpilot.impala.C}{0.013}
\@namedef{num@ctl.starpilot.impala.B_perm_mean}{0.003}
\@namedef{num@ctl.starpilot.impala.D_perm_mean}{0.002}
\@namedef{num@ctl.starpilot.impala.PR_train}{1.409}
\@namedef{num@ctl.starpilot.impala.z}{13.416}
\@namedef{num@ctl.starpilot.impala.A_over_B_permmean}{2.903}
\@namedef{num@ctl.starpilot.impala.C_over_D_permmean}{5.388}
\@namedef{num@ctl.starpilot.fpn.reported}{0.020}
\@namedef{num@ctl.starpilot.fpn.perm_mean}{0.002}
\@namedef{num@ctl.starpilot.fpn.analytic}{0.002}
\@namedef{num@ctl.starpilot.fpn.A}{0.014}
\@namedef{num@ctl.starpilot.fpn.C}{0.012}
\@namedef{num@ctl.starpilot.fpn.B_perm_mean}{0.003}
\@namedef{num@ctl.starpilot.fpn.D_perm_mean}{0.003}
\@namedef{num@ctl.starpilot.fpn.PR_train}{1.648}
\@namedef{num@ctl.starpilot.fpn.z}{14.757}
\@namedef{num@ctl.starpilot.fpn.A_over_B_permmean}{4.827}
\@namedef{num@ctl.starpilot.fpn.C_over_D_permmean}{3.970}
\@namedef{num@ctl.fruitbot.impala.reported}{0.144}
\@namedef{num@ctl.fruitbot.impala.perm_mean}{0.023}
\@namedef{num@ctl.fruitbot.impala.analytic}{0.023}
\@namedef{num@ctl.fruitbot.impala.A}{0.259}
\@namedef{num@ctl.fruitbot.impala.C}{0.251}
\@namedef{num@ctl.fruitbot.impala.B_perm_mean}{0.040}
\@namedef{num@ctl.fruitbot.impala.D_perm_mean}{0.039}
\@namedef{num@ctl.fruitbot.impala.PR_train}{22.578}
\@namedef{num@ctl.fruitbot.impala.z}{86.405}
\@namedef{num@ctl.fruitbot.impala.A_over_B_permmean}{6.426}
\@namedef{num@ctl.fruitbot.impala.C_over_D_permmean}{6.482}
\@namedef{num@ctl.fruitbot.fpn.reported}{0.042}
\@namedef{num@ctl.fruitbot.fpn.perm_mean}{0.008}
\@namedef{num@ctl.fruitbot.fpn.analytic}{0.008}
\@namedef{num@ctl.fruitbot.fpn.A}{0.081}
\@namedef{num@ctl.fruitbot.fpn.C}{0.097}
\@namedef{num@ctl.fruitbot.fpn.B_perm_mean}{0.015}
\@namedef{num@ctl.fruitbot.fpn.D_perm_mean}{0.014}
\@namedef{num@ctl.fruitbot.fpn.PR_train}{7.376}
\@namedef{num@ctl.fruitbot.fpn.z}{23.196}
\@namedef{num@ctl.fruitbot.fpn.A_over_B_permmean}{5.558}
\@namedef{num@ctl.fruitbot.fpn.C_over_D_permmean}{6.960}
\@namedef{num@ctl.z.min}{13}
\@namedef{num@ctl.z.max}{86}
\@namedef{num@ctl.fruitbot.collapse.min}{5.6}
\@namedef{num@ctl.fruitbot.collapse.max}{7.0}
\@namedef{num@d4.raw}{3.44}
\@namedef{num@d4.perm}{1.15}
\@namedef{num@d4.analytic}{1.14}
\@namedef{num@d4.analytic.s1}{1.18}
\@namedef{num@d4.analytic.s2}{0.95}
\@namedef{num@d4.analytic.s3}{1.48}
\@namedef{num@geo16.impala.reported}{0.48}
\@namedef{num@geo16.impala.factor}{4.6}
\@namedef{num@geo16.impala.published}{0.104}
\@namedef{num@geo16.fpn.reported}{0.43}
\@namedef{num@geo16.fpn.factor}{6.3}
\@namedef{num@geo16.fpn.published}{0.068}
\@namedef{num@geo16.collapse.min}{50}
\@namedef{num@geo16.collapse.max}{77}
\@namedef{num@geo.collapse.min}{4.1}
\@namedef{num@geo.collapse.max}{6.2}
\makeatother


==> numbers_cobbe.tex <==
% generated by scripts/tmlr_cobbe.py
\makeatletter
\@namedef{num@cobbe.mean.8M.sampled_train}{0.25}
\@namedef{num@cobbe.mean.8M.sampled_test}{0.19}
\@namedef{num@cobbe.mean.8M.greedy_test}{0.05}
\@namedef{num@cobbe.mean.8M.floor_test}{$-$0.07}
\@namedef{num@cobbe.mean.25M.sampled_train}{0.60}
\@namedef{num@cobbe.mean.25M.sampled_test}{0.33}
\@namedef{num@cobbe.mean.25M.greedy_test}{0.25}
\@namedef{num@cobbe.mean.25M.floor_test}{$-$0.03}
\@namedef{num@cobbe.starpilot.8M.sampled_train}{0.25}
\@namedef{num@cobbe.starpilot.8M.sampled_test}{0.26}
\@namedef{num@cobbe.starpilot.8M.greedy_test}{0.25}
\@namedef{num@cobbe.starpilot.8M.floor_test}{$-$0.01}
\@namedef{num@cobbe.fruitbot.8M.sampled_train}{0.76}
\@namedef{num@cobbe.fruitbot.8M.sampled_test}{0.72}
\@namedef{num@cobbe.fruitbot.8M.greedy_test}{0.81}
\@namedef{num@cobbe.fruitbot.8M.floor_test}{$-$0.03}
\@namedef{num@cobbe.bigfish.8M.sampled_train}{0.09}
\@namedef{num@cobbe.bigfish.8M.sampled_test}{0.05}
\@namedef{num@cobbe.bigfish.8M.greedy_test}{0.06}
\@namedef{num@cobbe.bigfish.8M.floor_test}{$-$0.00}
\@namedef{num@cobbe.coinrun.8M.sampled_train}{0.15}
\@namedef{num@cobbe.coinrun.8M.sampled_test}{0.14}
\@namedef{num@cobbe.coinrun.8M.greedy_test}{$-$0.29}
\@namedef{num@cobbe.coinrun.8M.floor_test}{$-$0.34}
\@namedef{num@cobbe.miner.8M.sampled_train}{0.52}
\@namedef{num@cobbe.miner.8M.sampled_test}{0.39}
\@namedef{num@cobbe.miner.8M.greedy_test}{$-$0.08}
\@namedef{num@cobbe.miner.8M.floor_test}{$-$0.03}
\@namedef{num@cobbe.dodgeball.8M.sampled_train}{0.01}
\@namedef{num@cobbe.dodgeball.8M.sampled_test}{$-$0.02}
\@namedef{num@cobbe.dodgeball.8M.greedy_test}{$-$0.04}
\@namedef{num@cobbe.dodgeball.8M.floor_test}{$-$0.06}
\@namedef{num@cobbe.bossfight.8M.sampled_train}{0.10}
\@namedef{num@cobbe.bossfight.8M.sampled_test}{0.07}
\@namedef{num@cobbe.bossfight.8M.greedy_test}{0.14}
\@namedef{num@cobbe.bossfight.8M.floor_test}{$-$0.03}
\@namedef{num@cobbe.heist.8M.sampled_train}{0.14}
\@namedef{num@cobbe.heist.8M.sampled_test}{$-$0.10}
\@namedef{num@cobbe.heist.8M.greedy_test}{$-$0.47}
\@namedef{num@cobbe.heist.8M.floor_test}{$-$0.05}
\@namedef{num@cobbe.starpilot.25M.sampled_train}{0.45}
\@namedef{num@cobbe.starpilot.25M.sampled_test}{0.41}
\@namedef{num@cobbe.starpilot.25M.greedy_test}{0.44}
\@namedef{num@cobbe.starpilot.25M.floor_test}{$-$0.01}
\@namedef{num@cobbe.fruitbot.25M.sampled_train}{0.84}
\@namedef{num@cobbe.fruitbot.25M.sampled_test}{0.66}
\@namedef{num@cobbe.fruitbot.25M.greedy_test}{0.72}
\@namedef{num@cobbe.fruitbot.25M.floor_test}{$-$0.03}
\@namedef{num@cobbe.heist.25M.sampled_train}{0.53}
\@namedef{num@cobbe.heist.25M.sampled_test}{$-$0.08}
\@namedef{num@cobbe.heist.25M.greedy_test}{$-$0.40}
\@namedef{num@cobbe.heist.25M.floor_test}{$-$0.05}
\makeatother


==> numbers_merged.tex <==
% generated by scripts/tmlr_merged_stats.py (exploratory)
\makeatletter
\@namedef{num@m.starpilot.test}{14.70}
\@namedef{num@m.starpilot.test.d}{13.03}
\@namedef{num@m.starpilot.test.lo}{11.19}
\@namedef{num@m.starpilot.test.hi}{14.93}
\@namedef{num@m.starpilot.test.ph}{$3.5\times10^{-4}$}
\@namedef{num@m.starpilot.test.label}{above floor}
\@namedef{num@m.starpilot.test.mg}{$-$3.20}
\@namedef{num@m.starpilot.test.mg.p}{0.12}
\@namedef{num@m.starpilot.test.ms}{$-$3.65}
\@namedef{num@m.starpilot.test.dis}{33}
\@namedef{num@m.starpilot.train}{14.67}
\@namedef{num@m.starpilot.train.d}{13.27}
\@namedef{num@m.starpilot.train.lo}{11.68}
\@namedef{num@m.starpilot.train.hi}{14.92}
\@namedef{num@m.starpilot.train.ph}{$1.5\times10^{-4}$}
\@namedef{num@m.starpilot.train.label}{above floor}
\@namedef{num@m.starpilot.train.mg}{$-$1.96}
\@namedef{num@m.starpilot.train.mg.p}{0.24}
\@namedef{num@m.starpilot.train.ms}{$-$3.45}
\@namedef{num@m.starpilot.train.dis}{34}
\@namedef{num@m.fruitbot.test}{26.07}
\@namedef{num@m.fruitbot.test.d}{28.74}
\@namedef{num@m.fruitbot.test.lo}{27.53}
\@namedef{num@m.fruitbot.test.hi}{30.05}
\@namedef{num@m.fruitbot.test.ph}{$9.2\times10^{-8}$}
\@namedef{num@m.fruitbot.test.label}{above floor}
\@namedef{num@m.fruitbot.test.mg}{0.28}
\@namedef{num@m.fruitbot.test.mg.p}{0.49}
\@namedef{num@m.fruitbot.test.ms}{3.19}
\@namedef{num@m.fruitbot.test.dis}{21}
\@namedef{num@m.fruitbot.train}{26.47}
\@namedef{num@m.fruitbot.train.d}{28.91}
\@namedef{num@m.fruitbot.train.lo}{28.32}
\@namedef{num@m.fruitbot.train.hi}{29.49}
\@namedef{num@m.fruitbot.train.ph}{$1.7\times10^{-19}$}
\@namedef{num@m.fruitbot.train.label}{above floor}
\@namedef{num@m.fruitbot.train.mg}{$-$0.21}
\@namedef{num@m.fruitbot.train.mg.p}{0.40}
\@namedef{num@m.fruitbot.train.ms}{2.37}
\@namedef{num@m.fruitbot.train.dis}{21}
\@namedef{num@m.bigfish.test}{2.67}
\@namedef{num@m.bigfish.test.d}{1.83}
\@namedef{num@m.bigfish.test.lo}{0.63}
\@namedef{num@m.bigfish.test.hi}{3.14}
\@namedef{num@m.bigfish.test.ph}{0.15}
\@namedef{num@m.bigfish.test.label}{not distinguishable}
\@namedef{num@m.bigfish.test.mg}{$-$0.52}
\@namedef{num@m.bigfish.test.mg.p}{0.084}
\@namedef{num@m.bigfish.test.ms}{$-$0.15}
\@namedef{num@m.bigfish.test.dis}{43}
\@namedef{num@m.bigfish.train}{4.05}
\@namedef{num@m.bigfish.train.d}{3.15}
\@namedef{num@m.bigfish.train.lo}{1.67}
\@namedef{num@m.bigfish.train.hi}{4.72}
\@namedef{num@m.bigfish.train.ph}{0.077}
\@namedef{num@m.bigfish.train.label}{not distinguishable}
\@namedef{num@m.bigfish.train.mg}{$-$0.58}
\@namedef{num@m.bigfish.train.mg.p}{0.17}
\@namedef{num@m.bigfish.train.ms}{$-$0.36}
\@namedef{num@m.bigfish.train.dis}{36}
\@namedef{num@m.coinrun.test}{2.71}
\@namedef{num@m.coinrun.test.d}{$-$0.57}
\@namedef{num@m.coinrun.test.lo}{$-$1.71}
\@namedef{num@m.coinrun.test.hi}{0.60}
\@namedef{num@m.coinrun.test.ph}{0.40}
\@namedef{num@m.coinrun.test.label}{not distinguishable}
\@namedef{num@m.coinrun.test.mg}{$-$0.86}
\@namedef{num@m.coinrun.test.mg.p}{0.005}
\@namedef{num@m.coinrun.test.ms}{$-$3.01}
\@namedef{num@m.coinrun.test.dis}{61}
\@namedef{num@m.coinrun.train}{2.86}
\@namedef{num@m.coinrun.train.d}{$-$0.09}
\@namedef{num@m.coinrun.train.lo}{$-$1.28}
\@namedef{num@m.coinrun.train.hi}{1.05}
\@namedef{num@m.coinrun.train.ph}{1.00}
\@namedef{num@m.coinrun.train.label}{not distinguishable}
\@namedef{num@m.coinrun.train.mg}{$-$0.90}
\@namedef{num@m.coinrun.train.mg.p}{$3.7\times10^{-4}$}
\@namedef{num@m.coinrun.train.ms}{$-$2.89}
\@namedef{num@m.coinrun.train.dis}{62}
\@namedef{num@m.miner.test}{0.47}
\@namedef{num@m.miner.test.d}{$-$0.70}
\@namedef{num@m.miner.test.lo}{$-$0.94}
\@namedef{num@m.miner.test.hi}{$-$0.47}
\@namedef{num@m.miner.test.ph}{$9.3\times10^{-6}$}
\@namedef{num@m.miner.test.label}{below floor}
\@namedef{num@m.miner.test.mg}{$-$0.13}
\@namedef{num@m.miner.test.mg.p}{0.010}
\@namedef{num@m.miner.test.ms}{$-$5.46}
\@namedef{num@m.miner.test.dis}{38}
\@namedef{num@m.miner.train}{1.11}
\@namedef{num@m.miner.train.d}{$-$0.13}
\@namedef{num@m.miner.train.lo}{$-$0.60}
\@namedef{num@m.miner.train.hi}{0.35}
\@namedef{num@m.miner.train.ph}{1.00}
\@namedef{num@m.miner.train.label}{not distinguishable}
\@namedef{num@m.miner.train.mg}{$-$0.10}
\@namedef{num@m.miner.train.mg.p}{0.056}
\@namedef{num@m.miner.train.ms}{$-$6.37}
\@namedef{num@m.miner.train.dis}{38}
\@namedef{num@m.dodgeball.test}{0.13}
\@namedef{num@m.dodgeball.test.d}{$-$0.34}
\@namedef{num@m.dodgeball.test.lo}{$-$0.47}
\@namedef{num@m.dodgeball.test.hi}{$-$0.20}
\@namedef{num@m.dodgeball.test.ph}{$5.0\times10^{-4}$}
\@namedef{num@m.dodgeball.test.label}{below floor}
\@namedef{num@m.dodgeball.test.mg}{$-$0.69}
\@namedef{num@m.dodgeball.test.mg.p}{$7.5\times10^{-5}$}
\@namedef{num@m.dodgeball.test.ms}{$-$0.96}
\@namedef{num@m.dodgeball.test.dis}{68}
\@namedef{num@m.dodgeball.train}{0.37}
\@namedef{num@m.dodgeball.train.d}{$-$0.20}
\@namedef{num@m.dodgeball.train.lo}{$-$0.41}
\@namedef{num@m.dodgeball.train.hi}{0.02}
\@namedef{num@m.dodgeball.train.ph}{0.44}
\@namedef{num@m.dodgeball.train.label}{not distinguishable}
\@namedef{num@m.dodgeball.train.mg}{$-$0.91}
\@namedef{num@m.dodgeball.train.mg.p}{$1.8\times10^{-5}$}
\@namedef{num@m.dodgeball.train.ms}{$-$1.32}
\@namedef{num@m.dodgeball.train.dis}{65}
\@namedef{num@m.bossfight.test}{1.18}
\@namedef{num@m.bossfight.test.d}{1.09}
\@namedef{num@m.bossfight.test.lo}{0.01}
\@namedef{num@m.bossfight.test.hi}{2.29}
\@namedef{num@m.bossfight.test.ph}{0.31}
\@namedef{num@m.bossfight.test.label}{not distinguishable}
\@namedef{num@m.bossfight.test.mg}{$-$1.10}
\@namedef{num@m.bossfight.test.mg.p}{$2.7\times10^{-4}$}
\@namedef{num@m.bossfight.test.ms}{$-$0.18}
\@namedef{num@m.bossfight.test.dis}{73}
\@namedef{num@m.bossfight.train}{1.48}
\@namedef{num@m.bossfight.train.d}{1.47}
\@namedef{num@m.bossfight.train.lo}{0.29}
\@namedef{num@m.bossfight.train.hi}{2.89}
\@namedef{num@m.bossfight.train.ph}{0.44}
\@namedef{num@m.bossfight.train.label}{not distinguishable}
\@namedef{num@m.bossfight.train.mg}{$-$1.29}
\@namedef{num@m.bossfight.train.mg.p}{0.031}
\@namedef{num@m.bossfight.train.ms}{$-$0.22}
\@namedef{num@m.bossfight.train.dis}{70}
\@namedef{num@m.heist.test}{0.08}
\@namedef{num@m.heist.test.d}{$-$3.07}
\@namedef{num@m.heist.test.lo}{$-$3.56}
\@namedef{num@m.heist.test.hi}{$-$2.60}
\@namedef{num@m.heist.test.ph}{$8.4\times10^{-26}$}
\@namedef{num@m.heist.test.label}{below floor}
\@namedef{num@m.heist.test.mg}{$-$0.37}
\@namedef{num@m.heist.test.mg.p}{0.016}
\@namedef{num@m.heist.test.ms}{$-$2.80}
\@namedef{num@m.heist.test.dis}{73}
\@namedef{num@m.heist.train}{0.18}
\@namedef{num@m.heist.train.d}{$-$3.36}
\@namedef{num@m.heist.train.lo}{$-$3.87}
\@namedef{num@m.heist.train.hi}{$-$2.87}
\@namedef{num@m.heist.train.ph}{$2.3\times10^{-28}$}
\@namedef{num@m.heist.train.label}{below floor}
\@namedef{num@m.heist.train.mg}{$-$0.98}
\@namedef{num@m.heist.train.mg.p}{$9.1\times10^{-4}$}
\@namedef{num@m.heist.train.ms}{$-$4.24}
\@namedef{num@m.heist.train.dis}{72}
\makeatother


==> tab_cka.tex <==
\begin{tabular}{llrrrr}
\toprule
& & \multicolumn{2}{c}{8M} & \multicolumn{2}{c}{25M} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Env & Comparison & Mean & SD & Mean & SD \\
\midrule
starpilot & IMPALA: train vs.\ test$^\ast$ & 0.020 & 0.001 & 0.022 & 0.004 \\
starpilot & FPN: train vs.\ test$^\ast$ & 0.020 & 0.007 & 0.021 & 0.009 \\
starpilot & cross-encoder, train & 0.703 & 0.063 & 0.757 & 0.065 \\
starpilot & cross-encoder, test & 0.731 & 0.038 & 0.783 & 0.058 \\
\addlinespace
fruitbot & IMPALA: train vs.\ test$^\ast$ & 0.144 & 0.012 & 0.110 & 0.012 \\
fruitbot & FPN: train vs.\ test$^\ast$ & 0.042 & 0.012 & 0.085 & 0.009 \\
fruitbot & cross-encoder, train & 0.543 & 0.026 & 0.518 & 0.022 \\
fruitbot & cross-encoder, test & 0.458 & 0.042 & 0.533 & 0.023 \\
\addlinespace
heist & IMPALA: train vs.\ test$^\ast$ & -- & -- & 0.104 & 0.024 \\
heist & FPN: train vs.\ test$^\ast$ & -- & -- & 0.068 & 0.009 \\
heist & cross-encoder, train & -- & -- & 0.593 & 0.048 \\
heist & cross-encoder, test & -- & -- & 0.678 & 0.041 \\
\bottomrule
\end{tabular}

